Can The Crowd Identify Misinformation Objectively? The Effects of Judgment Scale and Assessor's Background

Truthfulness judgments are a fundamental step in the process of fighting misinformation, as they are crucial to train and evaluate classifiers that automatically distinguish true and false statements. Usually such judgments are made by experts, like journalists for political statements or medical doctors for medical statements. In this paper, we follow a different approach and rely on (non-expert) crowd workers. This of course leads to the following research question: Can crowdsourcing be reliably used to assess the truthfulness of information and to create large-scale labeled collections for information credibility systems? To address this issue, we present the results of an extensive study based on crowdsourcing: we collect thousands of truthfulness assessments over two datasets, and we compare expert judgments with crowd judgments, expressed on scales with various granularity levels. We also measure the political bias and the cognitive background of the workers, and quantify their effect on the reliability of the data provided by the crowd.

==> 4-Analysis.tex.old.tex <==

\section{Results}\label{sec:res}
\subsection{Worker Background and Behavior}\label{sect:worker-questionnaire}
About six hundred US resident\footnote{MTurk workers based in the US must provide evidence they are eligible to work.}
crowd workers participated to this study on MTurk.
% 
% 
Across all experiments, 
the majority of workers (46.33\%) are between 26 and 35 years old. Second, workers in our study are well-educated as more than 60.84\% of workers have a four years college degree at least. Third, around 67.66\% of  workers earn less than \$75,000 a year. 


Nearly half (47.33\%) of the workers think their views are more democratic and only about 22.5\% of workers selected the Republican Party as voting preference. As for political views, Liberal and Moderate accounted for the most substantial proportion of workers, 29.5\% and 28.83\% respectively, while Very Conservative accounted for the least, only 5.67\%. In response to the border issue, 52.33\% of US-based workers  are against the construction of a wall on the southern border, while 36.5\% of the workers supported the building. For environmental protection, 80\% of the workers supported the government to strengthen environmental regulation to prevent climate change, while 11.33\% of the workers objected.

Based on the behavioral actions we logged as workers went through the HITs, Table \ref{tab:worker-behavior-data} shows the ratio of workers who completed the task, abandoned the task, and failed the quality checks.
Abandonment numbers are in line with previous studies \cite{8873609}. We can observe a higher failure and lower completion rate for \onehundred. This may show a slight lack of comfort for workers in using the most fine-grained scale.
We also logged worker behavior in terms of going back to previously seen statement (less than 5\% over all scales).

\begin{table}[tbp]
\caption{Worker behavior rates (percentage).}
 \label{tab:worker-behavior-data}
    \centering
    \begin{tabular}{l@{ }ccccccccc}
\toprule
& \textbf{Completion} & \textbf{Abandonment} & \textbf{Failure}\\
\midrule
\three & 35 & 53 & 12\\
\six & 33 & 52 & 14\\
\onehundred & 25 & 53 & 22\\
\bottomrule
\end{tabular}
\end{table}

\subsection{Crowdsourced  Score Distributions}\label{sect:score-distribution}

\begin{figure}[tbp]
  \centering
  \begin{tabular}{@{}c@{}c@{}c@{}}
   %s3
    \includegraphics[width=.33\linewidth]{S3_rawDistr_all.pdf}&
    \includegraphics[width=.33\linewidth]{S6_rawDistr_all.pdf}&
    \includegraphics[width=.33\linewidth]{S100_rawDistr_all.pdf}\\
    %
    \includegraphics[width=.33\linewidth]{S3_rawDistr_all_gold.pdf}&
    \includegraphics[width=.33\linewidth]{S6_rawDistr_all_gold.pdf}&
    \includegraphics[width=.33\linewidth]{S100_rawDistr_all_gold.pdf}\\
    %
    \includegraphics[width=.33\linewidth]{S3_aggDistr_all.pdf}&
    \includegraphics[width=.33\linewidth]{S6_aggDistr_all.pdf}&
    \includegraphics[width=.33\linewidth]{S100_aggDistr_all.pdf}\\
    
  \end{tabular}
\caption{%
    From left to right: \three, \six, \onehundred.
    From top to bottom: individual scores distribution (first row),
    gold scores distribution (second row), and
    aggregated scores distribution (third row). 
}
  \label{fig:scores_distributions}
\end{figure}


This section presents an analysis of score distributions obtained by the crowd for the statements used in our experiment.
% 
Figure~\ref{fig:scores_distributions} shows the distribution (and the cumulative distribution in red) for the individual scores provided by workers over the three crowd collections (i.e., \three, \six, and \onehundred) for \emph{all} the statements considered in the experiment; the behavior is similar across  \politifact and \abc statements (not shown because of space limitations).

The first row of the figure 
shows the raw score distributions for the three collections. As we can see from the plots, for all \three, \six, and \onehundred the distribution is skewed towards the right part of the scale representing higher truthfulness values; this can be also seen by looking at the cumulative distribution, which is steeper on the right hand side of the plots. 
It can also be seen that all three distributions are multimodal.
Looking at \onehundred we can  see a mild \emph{round number tendency}, that is, the tendency of workers to provide truthfulness scores which are multiple of 10 (35\% of \onehundred scores are multiple of 10; 23\% are 0, 50, or 100); such behavior was already noted by  \citet{Maddalena:2017:CRM:3026478.3002172}, \citet{RSDM:2018}, and \citet{Roitero:2018:FRS:3209978.3210052}. Also in this case, this behavior is consistent when considering separately \politifact and \abc documents (not shown).

%% GOLD
We now turn to \emph{gold} scores distribution, i.e., the special statements \high and \low that we used to perform  quality checks during the task. 
The second row of Figure~\ref{fig:scores_distributions} shows the scores distribution for the three crowd collections we considered. As we can see from the plots, the large majority of workers 
(44\% for \low and 45\% for \high in \three, 
34\% for \low and 39\% for \high in \six, and 
27\% for \low and 24\% for \high in \onehundred) 
provided as truthfulness level for these gold statements the extreme value of the scales (respectively the lower bound of the scale for \low and the upper bound of the scale for \high). This can be interpreted as a signal that the gathered data is of good quality. However, some workers provided judgments inconsistent with the gold labels. 

%% Aggregated
Finally, we discuss \emph{aggregated} scores. The third row of Figure~\ref{fig:scores_distributions} shows the score  distributions of \three, \six, and \onehundred judgments aggregated by taking the \emph{average} of the 10 scores obtained independently for each statement. 
As we can see from the plots, the distribution of the aggregated scores for all \three, \six, and \onehundred  are similar, they are no longer multimodal, and they are roughly bell-shaped.  
It is worth noting that, while the aggregated scores for \three (bottom-left plot in Figure \ref{fig:scores_distributions}) are skewed towards lower/negative --i.e., \abczero and \abcone-- scores, \three and \onehundred (bottom-mid and bottom-right plots in Figure \ref{fig:scores_distributions}) are skewed to higher/positive scores.  
This shows how different scales are used differently by the crowd.
As expected \cite{Maddalena:2017:CRM:3026478.3002172,RSDM:2018,Roitero:2018:FRS:3209978.3210052}, for \onehundred the round number tendency effect also disappears when judgments from different workers are aggregated together.
% 
In the following we discuss how  truthfulness scores gathered from the crowd compare to expert labels.



%Answering RQ2
\subsection{External and Internal Agreement}\label{sect:agreement-experts}

We now discuss the external agreement between the crowd judgments and the expert labels as well as the internal agreement among workers, addressing RQ2.


\begin{figure*}[tbp]
  \centering
  \begin{tabular}{@{}c@{}c@{}c@{}}
   %s3
    \includegraphics[width=.33\linewidth]{S3_truth_level_Scales_comparison_filter_all.pdf}&
    \includegraphics[width=.33\linewidth]{S6_truth_level_Scales_comparison_filter_all.pdf}&
    \includegraphics[width=.33\linewidth]{S100_truth_level_Scales_comparison_filter_all.pdf}\\
  \end{tabular}
\caption{%
    From left to right: \three, \six, \onehundred;
    agreement with \politifact and \abc, separated by the vertical dashed line. 
  \label{fig:scale-comparison-ground}}
\end{figure*}



\myparagraph{External Agreement.}
Figure~\ref{fig:scale-comparison-ground} shows the agreement between the aggregated crowd judgments and the ground truth (i.e., the expert labels provided for \politifact and \abc), for the \three, \six, and \onehundred crowd collections. As we can see from the plots, the behavior over all the three scales is similar, both on \politifact and \abc statements.
If we focus on \politifact documents (shown in the first panel of each plot), we can see that it is always the case that the \texttt{0} and \texttt{1} boxplot are very similar. This can point out a difficulty from workers to distinguish between the \politifactzero and \politifactone labels. The same behavior, even if less evident, is present between the \politifactone and \politifacttwo labels; this behavior is consistent across all the scales.
On the contrary, if we focus on the rest of the  \politifact labels, and on the \abc ones, we can see that the median lines of each boxplot are increasing while going towards labels representing higher truth values (i.e., going towards the right hand side of each chart), indicating that workers have higher agreement with the ground truth for those labels. Again, this behavior is consistent and similar for all the \three, \six, and \onehundred scales.


We measured the statistical significance of the differences between the ratings aggregated by mean for categories of the \six, \three, and \onehundred collections according to the Mann-Whitney rank test and the t-test. 
Concerning \abc, adjacent categories are significantly different in 5 cases out of 12, while the difference between non adjacent categories are all significant to the p$<.01$ level.
%
Concerning \politifact, the differences between the ratings aggregated by mean for adjacent categories and not adjacent ones by distance of 2 (e.g., \texttt{0} and \texttt{2})  are never significant with only one exception (distance 2);
differences for not adjacent categories of distance 3 are significant in 4/18 cases, and
differences for categories of distance 4 are significant in 5/12 of the cases.
Finally, categories of distance 5 (i.e., \texttt{0} and \texttt{5}) are significant in 4/6 cases.
% 
Although there is some signal, it is clear that the answer to RQ1 cannot be positive on the basis of this results. We will come back on this in Section \ref{sect:merge}.

\begin{figure}[tbp]
  \centering
  \begin{tabular}{@{}c@{}c@{}}
   %s3
    \includegraphics[width=.48\linewidth]{Agr_unitPairwise_with_Politifact_removeties.pdf} & 
    \includegraphics[width=.48\linewidth]{Agr_unitPairwise_with_ABC_removeties.pdf} \\
  \end{tabular}
\caption{%
    HIT pairwise agreement, relative frequency (\politifact on the left, \abc on the right).
  \label{fig:pairwise-unit-agreement}}
\end{figure}

\begin{figure}[tbp]
  \centering
  \begin{tabular}{@{}c@{}c@{}c@{}}
    %
    \includegraphics[width=.33\linewidth]{scatter_S6_vs_S3_Politifact.pdf}&
    \includegraphics[width=.33\linewidth]{scatter_S100_vs_S3_Politifact.pdf}&
    \includegraphics[width=.33\linewidth]{scatter_S100_vs_S6_Politifact.pdf}\\
    %
    \includegraphics[width=.33\linewidth]{scatter_S6_vs_S3_ABC.pdf}&
    \includegraphics[width=.33\linewidth]{scatter_S100_vs_S3_ABC.pdf}&
    \includegraphics[width=.33\linewidth]{scatter_S100_vs_S6_ABC.pdf}\\
  \end{tabular}
\caption{%
    Agreement between scales with a breakdown on \politifact statements (first row), and
    agreement between scales with a breakdown on \abc statements (second row).  From left to right: \six vs. \three, \onehundred vs. \three, and \onehundred vs. \six.  
  \label{fig:scale-comparisons}}
\end{figure}


We now turn on inspecting the agreement between the workers and the ground truth by looking at each HIT.
To do so, we computed, for all the \three, \six, and \onehundred collections the pairwise agreement \cite{10.1145/3121050.3121060} between the truthfulness scores expressed by workers and the ground truth labels, with a breakdown over \politifact and \abc statements.
We considered a slightly modified version of the pairwise agreement measure defined by \citet{10.1145/3121050.3121060}: in the attempt to make the pairwise agreement measure fully comparable across the different scales, we removed all the ties. 
% 
Intuitively, pairwise agreement as described in \citet{10.1145/3121050.3121060} measures the fraction of pairs in agreement between a ``ground truth'' scale and a ``crowd'' scale.
Specifically, a pair of crowd judgments (crowd-judgment$_1$, crowd-judgment$_2$) is considered to be in agreement if crowd-judgment$_1$ $\leq$ crowd-judgment$_2$ and the ground truth for crowd-judgment$_1$ is $<$ the ground truth for crowd-judgment$_2$. In our measurement\footnote{The code used to compute the pairwise agreement as defined by us can be found at \url{https://github.com/KevinRoitero/PairwiseAgreement}.} we removed all the ties (i.e., crowd-judgment$_1$ $=$ crowd-judgment$_2$), and we used $<$ in place of $\leq$. 
Figure~\ref{fig:pairwise-unit-agreement} shows the CCDF (Complementary Cumulative Distribution Function) of the relative frequencies of the HIT agreement. As we can see from the charts, the \three, \six, and \onehundred scales show a very similar level of external agreement; such behavior is consistent across the \politifact and \abc datasets. Again, this result confirms that all the considered scales present a similar level of external agreement with the ground truth, with the only exception of \onehundred  for the \abc dataset: this is probably due to the treatment of ties in the measure, that removes a different number of units for the three scales.

\myparagraph{Internal Agreement.}
We now turn to  investigate the internal agreement (i.e., the agreement measured among the workers themselves), and in particular we also compare workers using different scales. 
We computed a metric used to measure the level of agreement in a dataset, the Krippendorff's $\alpha$ \cite{krippendorff2011computing} coefficient. 
All $\alpha$ values within each of the three scales \three, \six, \onehundred and on both \politifact and \abc collections are in the $0.066$--$0.131$ range.
These results show that there is a rather low agreement among the workers \cite{krippendorff2011computing, checco2017let}.

To further investigate if the low agreement  we found depends on the specific scale used to label the statements, we  also performed all the possible transformations of judgments from one scale to another, following the methodology described by \citet{scale}. 
Figure~\ref{fig:scale-comparisons} shows the scatterplots, as well as the correlations, between the different scales on the \politifact and \abc statements. As we can see from the plots, the correlation values are around $\rho=0.55$--$0.6$ for \politifact and $\rho=0.35$--$0.5$ for \abc, for all the scales. The rank correlation coefficient $\tau$ is around $\tau=0.4$ for \politifact and $\tau=0.3$ for \abc. These values indicate a low correlation between all the scales; this is an indication that the same statements on different scales tend to be judged differently, both when considering their absolute value (i.e., $\rho$) and their relative ordering (i.e., $\tau$). 

\begin{figure}[tbp]
  \centering
  \begin{tabular}{@{}c@{}c@{}c@{}}
   %s3
    \includegraphics[width=.33\linewidth]{ALT_alpha_distr_S6to3.pdf} & 
    \includegraphics[width=.33\linewidth]{ALT_alpha_distr_S100to3.pdf} & 
    \includegraphics[width=.33\linewidth]{ALT_alpha_distr_S100to6.pdf}
  \end{tabular}
\caption{%
    From left to right: 
    \six cut into \three,
    \onehundred cut into \three, and
    \onehundred cut into \six (1\% stratified sampling), 
    cuts sorted by decreasing $\alpha$ values.
  \label{fig:alpha-cuts}}
\end{figure}

Figure~\ref{fig:alpha-cuts} shows the distribution of the $\alpha$ values when transforming one scale into another.\footnote{Note that the total number of possible cuts from \onehundred to \six is 75,287,520, thus we selected a sub-sample of all the possible cuts. We tried both \emph{stratified} and \emph{random} sampling, getting indistinguishable results.}
The dotted horizontal line in the plot represents $\alpha$ on the original dataset, the dashed line is the mean value of the (sampled) distribution.
% 
As we can see from the plots, values on the y-axis are very concentrated and all $\alpha$ values are close to zero ($[0,0.15]$ range). 
Thus, we can conclude that across all collections there is low level of internal agreement among workers, both within the same scale and across different scales. 


\subsection{Alternative Aggregation Functions}\label{sect:alternative-aggregation}

\begin{figure}[tbp]
  \centering
  \begin{tabular}{@{}c@{}c@{}c@{}}
   %s3
    \includegraphics[width=.33\linewidth]{S3_truth_level_Scales_comparison_filter_all_median.pdf}&
    \includegraphics[width=.33\linewidth]{S6_truth_level_Scales_comparison_filter_all_median.pdf}&
    \includegraphics[width=.33\linewidth]{S100_truth_level_Scales_comparison_filter_all_median.pdf}
  \end{tabular}
\caption{%
From left to right: \three, \six, \onehundred; agreement with ground truth.  Aggregation function: median (highlighted by the red diamond). Compare with Figure~\ref{fig:scale-comparison-ground}.
  \label{fig:alternative-aggregation-median}}
\end{figure}



\begin{figure}[tbp]
  \centering
  \begin{tabular}{@{}c@{}c@{}}
    %s3
    \includegraphics[width=.30\linewidth]{abc_verdict_simplified_vs_S3_truth_level_ABC_mvote.pdf}&
    \includegraphics[width=.49\linewidth]{politifact_label_vs_S3_truth_level_Politifact_mvote.pdf}\\
    %
    \includegraphics[width=.30\linewidth]{abc_verdict_simplified_vs_S6_truth_level_ABC_mvote.pdf}&
    \includegraphics[width=.49\linewidth]{politifact_label_vs_S6_truth_level_Politifact_mvote.pdf}
  \end{tabular}
\caption{%
    Agreement between \three (first row) and \six (second row), and 
    \abc (left) and \politifact (right). Aggregation function: mode.
  \label{fig:alternative-aggregration}}
\end{figure}

As anticipated in Section~\ref{sect:scales}, we also study the effect of aggregation functions alternative to the arithmetic mean. 
Figure~\ref{fig:alternative-aggregation-median} shows the results of using the \emph{median}: in this case the final truthfulness value for each statement has been computed by considering the median of the scores expressed by the workers. By comparing the charts to those in Figure~\ref{fig:scale-comparison-ground} it is clear that the median produces worst results.
The heatmaps in Figure~\ref{fig:alternative-aggregration} show the results  of using the \emph{majority vote} (i.e., the mode) as the alternative aggregation function. The mode is  more difficult to compare with the mean, but it is again clear that the overall quality is rather low: although the squares around the diagonal tend to be darker and contain higher values, there are many exceptions. These are mainly in the lower-left corners, indicating false positives, i.e., statements whose truth value is over-evaluated by the crowd; this tendency to false positives is absent with the mean (see Figure~\ref{fig:scale-comparison-ground}). Overall these results confirm that the choice of mean as aggregation function seems the most effective.

\subsection{Merging Assessment Levels}\label{sect:merge}

Given the result presented so far in Sections~\ref{sect:agreement-experts} and~\ref{sect:alternative-aggregation} (especially Figures~\ref{fig:scale-comparison-ground}, \ref{fig:alternative-aggregation-median}, and~\ref{fig:alternative-aggregration}, but also the rather low agreement and correlation values), the answer to RQ1 cannot be completely positive. There is a clear signal that aggregated values resemble the ground truth, but there are also several exceptions and statements that are mis-judged. However, there are some further considerations that can be made. First, results seem better for \abc  than \politifact. 
Second, it is not clear which specific scale should be used. The two expert collections used as ground truth use different scales, and we have experimented with the crowd on \three, \six, and \onehundred. Also, comparisons across different scales are possible, as we have shown above. Finally, a binary choice (true/false) seems also meaningful, and in many real applications it is what may really be needed.
Third, the above mentioned possible
confusion between \politifactzero and \politifactone suggest that these two categories could be fruitfully merged. This has 
been  done, for example, by \citet{tchechmedjiev2019claimskg}. 

All these remarks suggest to attempt some grouping of adjacent categories, to check if  by looking at the data on a more coarse-grained ground truth the results improve. Therefore, we group the six \politifact categories into either three (i.e., \texttt{01}, \texttt{23}, and \texttt{45}) or two (i.e., \texttt{012} and \texttt{345}) resulting ones, adopting the approach discussed by \citet{scale}. 
% 
Figure~\ref{fig:alternative-aggregation-binned-3} shows the results. The agreement with the ground truth can now be seen more clearly. The boxplots also seem quite well separated, especially when using the mean (the first three charts on the left). This is confirmed by analyses of statistical significance: all the differences in the boxplots on the bottom row are statistically significant at the p$<.01$ level for both t-test and Mann–Whitney, both with Bonferroni correction; the same holds for all the differences between \texttt{01} and \texttt{45} (the not adjacent categories) in the first row; for the other cases, i.e., concerning the adjacent categories,  further statistical significance is found at the  p<$.05$  level in 8 out of 24 possible cases. 

These results are much stronger than the previous ones: we can now state that the crowd is able to single out true from false statements with good accuracy; for statements with an intermediate degree of truthfulness/falsehood the accuracy is lower. 



\begin{figure}[tbp]
  \centering
  \begin{tabular}{@{}c@{}c@{}c@{}c@{}c@{}c@{}}
   %s3
    \includegraphics[width=.16\linewidth]{S3_truth_level_Scales_comparison_filter_all_bin3.pdf}&
    \includegraphics[width=.16\linewidth]{S6_truth_level_Scales_comparison_filter_all_bin3.pdf}&
    \includegraphics[width=.16\linewidth]{S100_truth_level_Scales_comparison_filter_all_bin3.pdf}&
    %
      \includegraphics[width=.16\linewidth]{S3_truth_level_Scales_comparison_filter_all_bin3_median.pdf}&
    \includegraphics[width=.16\linewidth]{S6_truth_level_Scales_comparison_filter_all_bin3_median.pdf}&
    \includegraphics[width=.16\linewidth]{S100_truth_level_Scales_comparison_filter_all_bin3_median.pdf}\\
    
      \includegraphics[width=.16\linewidth]{S3_truth_level_Scales_comparison_filter_all_bin2.pdf}&
    \includegraphics[width=.16\linewidth]{S6_truth_level_Scales_comparison_filter_all_bin2.pdf}&
    \includegraphics[width=.16\linewidth]{S100_truth_level_Scales_comparison_filter_all_bin2.pdf}&
    %
      \includegraphics[width=.16\linewidth]{S3_truth_level_Scales_comparison_filter_all_bin2_median.pdf}&
    \includegraphics[width=.16\linewidth]{S6_truth_level_Scales_comparison_filter_all_bin2_median.pdf}&
    \includegraphics[width=.16\linewidth]{S100_truth_level_Scales_comparison_filter_all_bin2_median.pdf}
  \end{tabular}
\caption{%
Agreement with ground truth for merged categories for \politifact. From the left:  mean for the three scales  \three, \six, \onehundred and then median for the same scales. From top to bottom: three  and two resulting categories. The median  is highlighted by the red diamond.
  \label{fig:alternative-aggregation-binned-3}}
\end{figure}

%Answering RQ3
\subsection{Sources of Evidence}\label{sect:justification-distribution}

\begin{table*}[tbp]
\caption{Websites from which workers chose URLs to justify their judgments without considering gold questions for \three, \six, and \onehundred (percentage). Only websites with percentage $\geq 1\%$ are shown.
    \label{tab:justification-distribution-sheet}}
    \centering
    \begin{tabular}{@{}l@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }c@{ }@{}}
\toprule
&  \footnotesize{Wikipedia} &   \footnotesize{Youtube} &   \footnotesize{The} &   \footnotesize{Factcheck} &  \footnotesize{Smh} &   \footnotesize{Cleveland} &   \footnotesize{Washington} &   \footnotesize{News} &   \footnotesize{Blogspot} &   \footnotesize{On the} &   \footnotesize{Quizlet} &   \footnotesize{NY} &   \footnotesize{CBS} &   \footnotesize{Forbes} &   \footnotesize{House} &   \footnotesize{Madison} &   \footnotesize{The} &   \footnotesize{Milwaukee} &   \footnotesize{Yahoo} \tabularnewline[-.5em]

 &  &   &   \footnotesize{Guardian} &    &   &    &  \footnotesize{Post}  &  &    &   \footnotesize{Issues} &    &  \footnotesize{Times} &   \footnotesize{News} &    &  & &   \footnotesize{Australian} &  \footnotesize{Journal}  &   \\
\midrule
\three  &      17 &    13 &        11 &       8 &  6 &       6 &            6 &  5 &      5 &         4 &     4 &     3 &      3 &    3 &   3 & 3 &           0 &      0 &   0 \\
\six   &      19 &    13 &        12 &       8 &  3 &       6 &            6 &  4 &      6 &         0 &     3 &     3 &      4 &   3 &   3 &     0 &           4 &      3 &   0 \\
\onehundred &      23 &    12 &        13 &       9 &  6 &       5 &            6 &  5 &      5 &         0 &     4 &     0 &      5 &    0 &   3 &     0 &           0 &      0 &   3 \\
\bottomrule
\end{tabular}
\end{table*}

Table~\ref{tab:justification-distribution-sheet} shows the distribution of websites used by workers to justify the truthfulness label they chose for each statement.
As we can see, the most used sources are, for all the scales, ``Wikipedia'' and ``YouTube'', followed by popular news websites such as ``The Guardian'' and  ``The Washington Post''. Furthermore, we can see that among the most popular sources there is one fact checking website (i.e., FactCheck). Noting that we intentionally removed \url{abc.com.au} and \url{politifact.com} URLs from those which could be selected, this shows that workers, supported by the search engine, tend to identify trustworthy information sources to support their judgment decisions.


\begin{table}[tbp]
\caption{Distribution of the ranks in search results for the URLs chosen by workers in \three, \six,  and \onehundred (percentage).}
 \label{tab:justification-distribution-rank}
    \centering
    \begin{tabular}{l@{ }ccccccccccc}
\toprule
& \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} & \textbf{9} & \textbf{10} & \textbf{11}\\
\midrule
\three          & 17 & 12 & 13 & 14 & 12 & 9  & 7 & 6 & 4 & 3 & 1\\
\six            & 13 & 13 & 16 & 12 & 11 & 9  & 8 & 7 & 5 & 4 & 1\\
\onehundred     & 15 & 15 & 15 & 12 & 8  & 12 & 7 & 6 & 5 & 2 & 1\\
\midrule
avg             & 15 & 13 & 15 & 11 & 10 & 10 & 7 & 6 & 5 & 3 & 1 \\
\bottomrule
\end{tabular}
\end{table}

Table~\ref{tab:justification-distribution-rank} 
shows the distribution of the ranks within the search engine results of the URLs chosen by workers to justify their judgments (without considering the gold questions), for \three, \six and \onehundred.
As we can see from the table, the majority of workers tend to click on the first results shown by the search engine, as expected \cite{kelly2015how,craswell2008experimental,joachims2017accurately}.
Nevertheless, the results also show that workers explore the first ten documents as ranked by the search engine and do not simply click on the first returned URL, thus putting some effort to find a reliable source and/or justification.
Finally, we note that over all the scales, all the workers stopped at the first page of results as returned by the search engine, and no one investigated search results with rank greater than 10.


%Answers RQ4
\subsection{Effect of Worker  Background and Bias} \label{sect:worker-bias}

\begin{table}[tbp]
\centering
\caption{Correlation between Cognitive Reflection Test (CRT) performance and z-scores for each scale level and the correlation between worker age and z-scores.
}
\label{tab:Correlation }
\begin{threeparttable}

\begin{tabular}{llSS}
\toprule
{\textbf{Dataset}}          & {\begin{tabular}[c]{@{}c@{}}\textbf{Correlation} \\ \textbf{with}\end{tabular}}            & {\textbf{Age}}                        & {\begin{tabular}[c]{@{}c@{}}\textbf{CRT} \\ \textbf{Performance}\end{tabular}} \\ \midrule
\multirow{4}{*}{\politifact}                                          & Pants-on-fire & -0.038                     & -0.098$^{\ast}$                                                       \\
                                                                     & False         & -0.022                      & -.072                                      \\
                                                                     & True          & .127$^{\ast} $ & 0.062                                                       \\
                                                                     & Discernment   & .113$^{\ast\ast} $ & .128$^{\ast\ast}$                                  \\
                                                                     \midrule
\multirow{3}{*}{\abc
} & Negative      & -0.075                      & -0.021                                                      \\
                                                                     & Positive      & 0.048                       & .11$^{\ast\ast}$                                 \\
                                                                     & Discernment   & 0.088$^\ast $      & .11$^{\ast\ast}$                                  \\
                                                                     \midrule
Total                                                                & Discernment   & .125$^{\ast\ast}$  & .154$^{\ast\ast}$                                  \\ \bottomrule
\end{tabular}
\begin{tablenotes}
{\small 
\item $^{\ast\ast}$: $p < 0.01 $, $^\ast$: $p <0.05$.
}
\end{tablenotes}
\end{threeparttable}

\end{table}
\myparagraph{CRT Test.}
To answer RQ4, we aim to assess the relationships that exists between workers' background and their performance.
In terms of workers' cognitive skills, we measure CRT performance as the percentage of correct answers given by them. Thus, a higher CRT score is associated to higher  analytical thinking ability~\cite{Frederick2005}.
% 
We compare worker performances across the three scales by means of the standardized calculation of the  $z$-score for each worker and each assessment level.
% 
The $z$-score for each statement represents the performance of crowd workers as compared to others.
% 
The lower the $z$-score for false statements, the stronger the ability of the crowd to identify lies and the higher the $z$-score for true statements, the higher the ability to identify accurate information.
``Discernment'' is then calculated by deducting the $z$-score for false statements from the $z$-score for true statements. This represents the ability of the crowd to distinguish the true from the false~\cite{pennycook2019lazy}.
% 
In this analysis we focus on statements with extreme true or false ground truth labels and discard the `in-between' statements as they do not provide additional evidence on the ability of the crowd to distinguish between true/false information.


Table~\ref{tab:Correlation } shows the results.
First, there is a statistically significant (Spearman's rank-order test), moderate positive correlation between Discernment and CRT score on statements from \politifact and \abc ($r_s(598)= 0.128$, $p = 0.002$ and $r_s(598)= 0.11$, $p = 0.007$ respectively).
% 
This shows that  workers who reflect more perform 
better in identifying pants-on-fire statements of US (local) politicians ($r_s(598)= -0.098$, $p = 0.017$), and identifying true statements of AU (not local) politicians ($r_s(598)= 0.11$, $p = 0.007$).
% 
In general, people with strong analytical abilities (as determined by the CRT test) can better recognize true statements from false($r_s(598)= 0.154$, $p<0.0005$).
% 
Besides, the ability to distinguish true from false increases with age ($r_s(598)= 0.125$, $ p=0.002$).
Older workers perform better in recognizing true statements by US politicians ($r_s(598)= 0.127$, $p=0.02$). 
The level of education and income do not have statistically significant correlation with their judgments.



\myparagraph{Political Background.}
%
% 
% 
As a Shapiro-Wilk test  ~\cite{shapiro1972approximate} confirms that discernment scores are normally distributed ($p > 0.05$) for groups with diverse political views, we can conducted a one-way ANOVA analysis to determine if the ability to distinguish true from false statements was different across groups.\footnote{As a Levene's Test ~\cite{schultz1985levene} showed that the homogeneity of variances was violated ($p = 0.034$) we used the Welch-Satterthwaite correction ~\cite{satterthwaite1946approximate}  to calculate the degrees of freedom and a Games-Howell post-hoc test ~\cite{ruxton2008time}  to show multiple comparisons.}
% 
Discernment score is statistically significantly different between different political views (Welch's $F(4, 176.735) = 3.451$, $p = 0.01$).
A Games-Howell post-hoc test confirms that the increase of discernment score (\num{0.453}, 95\% CI (\num{0.028} to \num{0.879}))  from conservative (\num{-0.208} ± \num{1.293}) to liberal (\num{0.245} ± \num{1.497}) is statistically significant ($p = 0.03$).
% 
Given these results, we can conclude that crowd workers who have liberal views can better differentiate between false and true statements. Furthermore, there is no statistically significant difference (we use a Kruskal-Wallis H tests ~\cite{kruskal1952use} as Shapiro-Wilk test ~\cite{shapiro1972approximate} $p < 0.05$) in discernment scores based on the political party in which crowd workers explicitly identified themselves with ($x^2(3)= 3.548$, $ p= 0.315$).
This shows there is no difference in judgment quality based on their explicit political stance.
However, an analysis of their implicit political views rather than their explicit party identification shows a different result.


From the above results we can see that while the explicit party identification does not have a significant impact on the judgment quality for true and false statements,  their implicit political orientation does. 
% 
The partisan gap on the immigration issue is apparent in the US. According to the survey conducted by Pew Research Center
in January 2019, about 82\% of Republicans and Republican-leaning independents support developing the barrier along the southern border of the United States, while 93\% of Democrats and Democratic leaners oppose it.
% The other most apparent partisan divide is on the environment problem, especially on climate change. 
Therefore, asking workers' opinion on this matter can be a way to know their implicit political orientation. 

 We use a Kruskal-Wallis H tests ~\cite{kruskal1952use} as Shapiro-Wilk test~\cite{shapiro1972approximate} ($p < 0.05$) in assessor's discernment between immigration policy groups defined based on their answer to the wall question. We observed statistically significant differences on Politifact statements ($x_2 (2) = 10.965, p = 0.004$) and on all statements ($x_2 (2) = 11.966, p = 0.003$).
% 
A post-hoc analysis using Dunn's procedure with a Bonferroni correction ~\cite{dunn1964multiple} revealed statistically significant differences in discernment scores on \politifact statements between agreeing (\num{-0.335}) and disagreeing (\num{0.245}) ($p = 0.007$) on building a wall. 
% 
Similar results are obtained when discernment scores are compared on all statement, there were statistically significant differences in discernment scores between agreeing (\num{-0.377}) and disagreeing (\num{0.173}) ($p = 0.002$) on building a wall along the southern border of the United States. 
% 
These results show how, in our experiment, crowd workers who do not want a wall on the southern US border perform better in distinguishing between true and false statements.
% 
We did not observe significant differences based on their stance on climate issues.

